M$^2$BEV: Multi-Camera Joint 3D Detection and Segmentation with Unified Birds-Eye View Representation

In this paper, we propose M$^2$BEV, a unified framework that jointly performs 3D object detection and map segmentation in the Birds Eye View~(BEV) space with multi-camera image inputs. Unlike the majority of previous works which separately process detection and segmentation, M$^2$BEV infers both tasks with a unified model and improves efficiency. M$^2$BEV efficiently transforms multi-view 2D image features into the 3D BEV feature in ego-car coordinates. Such BEV representation is important as it enables different tasks to share a single encoder. Our framework further contains four important designs that benefit both accuracy and efficiency: (1) An efficient BEV encoder design that reduces the spatial dimension of a voxel feature map. (2) A dynamic box assignment strategy that uses learning-to-match to assign ground-truth 3D boxes with anchors. (3) A BEV centerness re-weighting that reinforces with larger weights for more distant predictions, and (4) Large-scale 2D detection pre-training and auxiliary supervision. We show that these designs significantly benefit the ill-posed camera-based 3D perception tasks where depth information is missing. M$^2$BEV is memory efficient, allowing significantly higher resolution images as input, with faster inference speed. Experiments on nuScenes show that M$^2$BEV achieves state-of-the-art results in both 3D object detection and BEV segmentation, with the best single model achieving 42.5 mAP and 57.0 mIoU in these two tasks, respectively.

==> tables/gfl_test.tex <==
\begin{subtable}[ht]{0.29\textwidth}
	\begin{center}
		\captionsetup{font={scriptsize}}
	    \caption{Accuracy as a function of the MLP dimension $C$ in the decoder on ADE20K.}
	    \vspace{-4pt}
		\setlength{\tabcolsep}{2mm}
		\resizebox{\textwidth}{!}{
		\begin{tabular}{l | c c c}
            \toprule
            \multicolumn{1}{c|}{$C$} & Flops $\downarrow$  & Params $\downarrow$  & mIoU $\uparrow$  \\ \midrule
            256 & 25.7 & 24.7 & 44.9 \\ %\hline
            512 & 39.8 & 25.8 & 45.0 \\ %\hline
            768 & 62.4 & 27.5 & 45.4 \\ %\hline
            1024 & 93.6 & 29.6 & 45.2 \\% \hline
            2048 & 304.4 & 43.4 & 45.6 \\ \bottomrule
            \end{tabular}
		}
	    \label{tab:mlpdim}
	\end{center}
\end{subtable}
\hspace{2pt}
\begin{subtable}[ht]{0.32\textwidth}
	\begin{center}
		\captionsetup{font={scriptsize}}
		\caption{Mix-FFN vs. positional encoding (PE) for different test resolution on Cityscapes.}
		%\caption{Accuracy as a function of using Mix-FFN or a positional encoding (PE) for different test resolution on Cityscapes. For training we used 768$\times$768 image crops.}
		\vspace{-4pt}
		\setlength{\tabcolsep}{2mm}
		\resizebox{\textwidth}{!}{
    		\begin{tabular}{l c c}
            \toprule
                \begin{tabular}[c]{@{}c@{}}Inf Res\end{tabular} & \begin{tabular}[c]{@{}c@{}}Enc Type\end{tabular} & mIoU $\uparrow$ \\ \midrule
                768$\times$768 & PE    & 77.3  \\ %\hline
                1024$\times$2048 & PE    &74.0\\%~(-3.3)  \\ %\hline
                768$\times$768 & Mix-FFN    &  80.5\\ %\hline
                1024$\times$2048 & Mix-FFN    & 79.8\\%~(-0.7) \\
            \bottomrule
        \end{tabular}
		}
		\label{tab:resolution}
	\end{center}
\end{subtable}
% 
\hspace{2pt}
\begin{subtable}[ht]{0.29\textwidth}
	\begin{center}
		\captionsetup{font={scriptsize}}
	    \caption{Accuracy on ADE20K of CNN and Transformer encoder with MLP decoder. ``S4'' means stage-4 feature.}
	    \vspace{-4pt}
		\setlength{\tabcolsep}{1.0mm}
		\resizebox{\textwidth}{!}{
		\begin{tabular}{l c c c}
            \toprule
            \multicolumn{1}{l}{Encoder} & Flops $\downarrow$ & Params $\downarrow$ & mIoU $\uparrow$ \\ \midrule
            ResNet50~(S1-4)   & 69.2 & 29.0 & 34.7 \\ 
            ResNet101~(S1-4)  & 88.7 & 47.9 & 38.7 \\ 
            ResNeXt101~(S1-4)  & 127.5 & 86.8 & 39.8 \\ 
            \textbf{MiT-B2~(S4)}     & \textbf{22.3} & \textbf{24.7} & 43.1 \\
            \textbf{MiT-B2 (S1-4)}     & 62.4 & 27.7 & 45.4 \\ 
            \textbf{MiT-B3 (S1-4)}     & 79.0 & 47.3 & \textbf{48.6} \\ \bottomrule
            \end{tabular}
		}
	    \label{tab:cnnencoder}
	\end{center}
\end{subtable}
\hspace{5pt}

